Learning in memristive electrical circuits

Memristors are nonlinear two-terminal circuit elements whose resistance at a given time depends on past electrical stimuli. Recently, networks of memristors have received attention in neuromorphic computing since they can be used as a tool to perform linear algebraic operations, like matrix-vector multiplication, directly in hardware. In this paper, the aim is to resolve two fundamental questions pertaining to a specific, but relevant, class of memristive circuits called crossbar arrays. In particular, we show (1) how the resistance values of the memristors at a given time can be determined from external (voltage and current) measurements, and (2) how the resistances can be steered to desired values by applying suitable external voltages to the network. The results will be applied to solve a prototypical learning problem, namely linear least squares, by applying and measuring voltages and currents in a suitable memristive circuit.

==> References/references.tex <==
\bibitem{Ribar2021} L. Ribar and R. Sepulchre. ``Neuromorphic control: Designing Multiscale Mixed-Feedback Systems." \textit{IEEE Control Syst. Mag.} 41(6), pp. 34--63, 2021.

\bibitem{Indiveri2015} G. Indiveri and S.-C. Liu. ``Memory and Information Processing in Neuromorphic Systems”.  \textit{Proc. IEEE} 103(8), pp. 1379–-1397, 2015.

\bibitem{Mead1990} C. Mead. ``Neuromorphic electronic systems”. \textit{Proc. IEEE} 78(10), pp. 1629--1636, 1990.

\bibitem{Thomas2013} A. Thomas. ``Memristor-based neural networks”.  \textit{J. Phys. D Appl. Phys.} 46(9), pp. 093001, 2013.

\bibitem{Snider2011} G. Snider et al. ``From Synapses to Circuitry: Using Memristive Memory to Explore the Electronic Brain". \textit{Computer}, 44(2), pp. 21--28, 2011.

\bibitem{Khalid2019} M. Khalid. ``Review on Various Memristor Models, Characteristics, Potential Applications, and Future Works." \textit{Trans. electr. electron. mater.} 20, pp. 289--298, 2019.

\bibitem{Sah2014}
M.P. Sah et al. ``Brains Are Made of Memristors." \textit{IEEE Circ. Syst. Mag.} 14(1), pp. 12--36, 2014.

\bibitem{Chua1971} L. Chua. ``Memristor-The missing circuit element”.  \textit{IEEE Trans. Circ. Theory} 18(5), pp. 507–519, 1971.


\bibitem{Corinto2016} F. Corinto and M. Forti. ``Memristor Circuits: Flux—Charge Analysis Method”.  \textit{IEEE Trans. Circuits Syst. I: Regul. Pap.} 63(11), pp. 1997–-2009, 2016.

\bibitem{Corinto2021} F. Corinto et al. Nonlinear Circuits and Systems with Memristors. Springer, 2021.

\bibitem{Chaffey2024} T. Chaffey and R. Sepulchre. ``Monotone One-Port Circuits." \textit{IEEE Trans. Automat. Contr.} 69(2), pp. 783--796, 2024.

\bibitem{Corinto2015} F. Corinto et al. ``A Theoretical Approach to Memristor Devices." \textit{IEEE J. Emerg. Sel. Top. Circuits Syst.} 5(2), pp. 123--132, 2015.

\bibitem{Huijzer2023} M.A. Huijzer et al. ``Synchronisation in Electrical Circuits With Memristors and Grounded Capacitors." \textit{IEEE Control Syst. Lett.} 7, pp. 1849--1854, 2023.

\bibitem{Sun2019} Z. Sun et al. ``Solving matrix equations in one step with cross-point resistive arrays”. In:  \textit{PNAS USA} 116(10), pp. 4123--4128, 2019.

\bibitem{Sebastian2020} A. Sebastian et al. ``Memory devices and applications for in-memory computing”.  \textit{Nat. Nanotechnol.} 15(7), pp. 529--544, 2020.

\bibitem{Strukov2008} Strukov, D. B., et al. ``The missing memristor found." \textit{nature} 453.7191 (2008): 80-83.
 

\bibitem{Pates2019} R. Pates et al. ``On the Optimal Control of Relaxation Systems."  \textit{IEEE CDC}, pp. 6068 -- 6073, 2019.


